A Bit-Parallel Russian Dolls Search for a Maximum Cardinality Clique in a Graph

Finding the clique of maximum cardinality in an arbitrary graph is an NP-Hard problem that has many applications, which has motivated studies to solve it exactly despite its difficulty. The great majority of algorithms proposed in the literature are based on the Branch and Bound method. In this paper, we propose an exact algorithm for the maximum clique problem based on the Russian Dolls Search method. When compared to Branch and Bound, the main difference of the Russian Dolls method is that the nodes of its search tree correspond to decision subproblems, instead of the optimization subproblems of the Branch and Bound method. In comparison to a first implementation of this Russian Dolls method from the literature, several improvements are presented. Some of them are adaptations of techniques already employed successfully in Branch and Bound algorithms, like the use of approximate coloring for pruning purposes and bit-parallel operations. Two different coloring heuristics are tested: the standard greedy and the greedy with recoloring. Other improvements are directly related to the Russian Dolls scheme: the adoption of recursive calls where each subproblem (doll) is solved itself via the same principles than the Russian Dolls Search and the application of an elimination rule allowing not to generate a significant number of dolls. Results of computational experiments show that the algorithm outperforms the best exact combinatorial algorithms in the literature for the great majority of the dense graphs tested, being more than twice faster in several cases.

==> nenem-leaves-dimacs.tex <==

\rowcolor[gray]{.8}  & 169.0 & 38.23 & 164.3 & 36.59 & -- & 0.141 & 0.140 & -- \\* 
\rowcolor[gray]{.8}  & 142.6 & 30.01 & 139.0 & 28.70 & -- & 0.165 & 0.164 & -- \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 176.7 & 37.97 & 174.1 & 37.20 & 0.506 & 0.146 & 0.147 & -- \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt p\_hat1000-1}  & 151.9 & 30.31 & 149.7 & 29.58 & 0.584 & 0.171 & 0.172 & -- \\
\hline

 & 1056 & 147.8 & 1451 & 229.1 & 5.55 & 1.30 & 1.65 & $\circ$ \\* 
 & 951.1 & 125.7 & 1377 & 220.1 & 4.25 & 1.51 & 1.87 & $\circ$ \\*
\cline{2-9}
 & 1487 & 220.6 & 1128 & 175.6 & 5.08 & 1.70 & 1.36 & $\star$ \\* 
\multirow{-4}{*}{\tt p\_hat1500-1}  & 1398 & 205.9 & 1033 & 154.6 & 5.44 & 1.93 & 1.63 & $\star$ \\
\hline

\rowcolor[gray]{.8}  & 22973 & 6017 & 13559 & 3451 & 2653 & 77.43 & 48.64 & $\star$$\star$ \\* 
\rowcolor[gray]{.8}  & 14598 & 3305 & 8690 & 1899  & 240.8 & 80.93 & 50.65 & $\star$$\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 39574 & 11504 & 20594 & 5789 & 284.1 & 127.7 & 71.43 & $\star$$\star$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt p\_hat1000-2}  & 24645 & 6402 & 12895 & 3217 & 245.7 & 133.3 & 74.08 & $\star$$\star$ \\
\hline

 & 76070 & 16081 & 74259 & 15532 & 441.4 & 87.69 & 88.53 & -- \\* 
 & 70427 & 15331 & 68479 & 14768 & 319.3 & 96.28 & 96.12 & -- \\*
\cline{2-9}
 & 79916 & 16289 & 82514 & 16969 & 295.4 & 92.39 & 96.76 & -- \\* 
\multirow{-4}{*}{\tt DSJC1000.5}  & 74569 & 15578 & 76987 & 16257 & 333.8 & 100.9 & 104.6 & -- \\
\hline

\rowcolor[gray]{.8}  & 1084 & 275.7 & 1012 & 255.9 & 4.57 & 0.774 & 0.764 & -- \\* 
\rowcolor[gray]{.8}  & 846.3 & 193.8 & 779.7 & 173.3 & 3.37 & 0.951 & 0.915 & -- \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 1183 & 287.7 & 1102 & 266.0 & 2.13 & 0.846 & 0.838 & -- \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt DSJC500.5}  & 950.5 & 211.8 & 874.3 & 189.3 & 2.51 & 1.03 & 0.998 & -- \\
\hline

 & 231.3 & 57.09 & 231.3 & 57.09 & 48.39 & 0.738 & 0.769 & -- \\* 
 & 162.5 & 33.74 & 162.5 & 33.74 & 6.10 & 0.839 & 0.856 & -- \\*
\cline{2-9}
 & 741.3 & 207.9 & 345.5 & 95.32 & 5.30 & 2.10 & 1.09 & $\star$$\star$ \\* 
\multirow{-4}{*}{\tt p\_hat700-2}  & 504.8 & 123.7 & 238.6 & 57.25 & 5.08 & 2.39 & 1.23 & $\star$$\star$ \\
\hline

\rowcolor[gray]{.8}  & 250.9 & 62.11 & 236.2 & 57.57 & -- & 0.175 & 0.174 & -- \\* 
\rowcolor[gray]{.8}  & 196.9 & 39.25 & 185.3 & 34.02 & -- & 0.216 & 0.207 & -- \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 266.0 & 63.91 & 204.4 & 44.12 & 0.433 & 0.185 & 0.159 & $\star$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt sanr400\_0.5}  & 212.7 & 41.94 & 164.0 & 26.29 & 0.520 & 0.230 & 0.190 & $\star$ \\
\hline

 & 1924228 & 451474 & 3544359 & 904788 & 19390 & 2975 & 5194 & $\circ$$\circ$ \\* 
 & 1327872 & 277754 & 2488522 & 600952 & 10188 & 3073 & 5321 & $\circ$$\circ$ \\*
\cline{2-9}
 & 2149229 & 487116 & 3891822 & 964831 & 9303 & 3367 & 5673 & $\circ$$\circ$ \\* 
\multirow{-4}{*}{\tt brock800\_1}  & 1546067 & 316388 & 2861531 & 682516 & 9497 & 3491 & 5901 & $\circ$$\circ$ \\
\hline

\rowcolor[gray]{.8}  & 1654952 & 387936 & 4459555 & 1155932 & 17492 & 2599 & 6448 & $\circ$$\circ$$\circ$ \\* 
\rowcolor[gray]{.8}  & 1172568 & 251211 & 3189649 & 806701 & 9121 & 2679 & 6636 & $\circ$$\circ$$\circ$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 2063020 & 474353 & 4460120 & 1118033 & 8533 & 3200 & 6388 & $\circ$$\circ$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt brock800\_2}  & 1522715 & 326797 & 3325413 & 816754 & 8378 & 3338 & 6700 & $\circ$$\circ$$\circ$ \\
\hline

 & 1065164 & 240368 & 1912833 & 464107 & 11829 & 1719 & 2968 & $\circ$$\circ$ \\* 
 & 757036 & 159313 & 1299528 & 280306  & 6272 & 1774 & 3013 & $\circ$$\circ$ \\*
\cline{2-9}
 & 1228395 & 269984 & 1951966 & 454995 & 5574 & 1973 & 3051 & $\circ$$\circ$ \\* 
\multirow{-4}{*}{\tt brock800\_3}  & 909264 & 187194 & 1395656 & 295756 & 5396 & 2068 & 3135 & $\circ$$\circ$ \\
\hline

\rowcolor[gray]{.8}  & 679270 & 145266 & 2833636 & 734803 & 8217 & 1171 & 4082 & $\circ$$\circ$$\circ$ \\* 
\rowcolor[gray]{.8}  & 480282 & 96096 & 1996967 & 497131  & 4356 & 1200 & 4261 & $\circ$$\circ$$\circ$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 2242760 & 536283 & 2641180 & 649939 & 3987 & 3315 & 3886 & $\circ$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt brock800\_4}  & 1695941 & 403075 & 1935412 & 458605 & 3913 & 3475 & 4096 & $\circ$ \\
\hline

 & 55258 & 16573 & 55275 & 16581 & 413.1 & 55.48 & 57.18 & -- \\* 
 & 35267 & 9666 & 35240 & 9656  & 197.2 & 64.46 & 64.91 & -- \\*
\cline{2-9}
 & 64523 & 18819 & 67641 & 19935 & 129.9 & 64.34 & 68.74 & $\circ$ \\* 
\multirow{-4}{*}{\tt sanr400\_0.7}  & 43415 & 11697 & 45552 & 12459 & 139.1 & 75.22 & 79.03 & -- \\
\hline

\rowcolor[gray]{.8}  & 407.5 & 127.4 & 154.2 & 44.19 & 11.77 & 0.607 & 0.260 & $\star$$\star$$\star$ \\* 
\rowcolor[gray]{.8}  & 243.8 & 69.22 & 93.78 & 22.74 & 2.72 & 0.758 & 0.317 & $\star$$\star$$\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 762.1 & 258.4 & 242.7 & 75.07 & 1.79 & 1.07 & 0.402 & $\star$$\star$$\star$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt p\_hat300-3}  & 458.6 & 142.7 & 149.9 & 40.95 & 1.94 & 1.36 & 0.489 & $\star$$\star$$\star$ \\
\hline

 & 307.2 & 101.7 & 460.0 & 160.5 & 1.87 & 0.214 & 0.312 & $\circ$ \\* 
 & 181.7 & 54.92 & 271.5 & 86.64 & 0.937 & 0.286 & 0.424 & $\circ$ \\*
\cline{2-9}
 & 391.0 & 129.2 & 482.5 & 164.6 & 0.495 & 0.269 & 0.328 & $\circ$ \\* 
\multirow{-4}{*}{\tt brock200\_1}  & 254.1 & 77.52 & 306.3 & 95.91 & 0.546 & 0.365 & 0.456 & $\circ$ \\
\hline

\rowcolor[gray]{.8}  & 178635 & 53031 & 218166 & 66623 & 1930 & 216.6 & 265.8 & $\circ$ \\* 
\rowcolor[gray]{.8}  & 104981 & 29024 & 123173 & 34472 & 755.3 & 237.4 & 284.9 & $\circ$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 203454 & 58646 & 182531 & 52453 & 495 & 245.5 & 232.4 & $\star$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt brock400\_1}  & 127091 & 34221 & 109789 & 28684 & 501.5 & 276.4 & 251.2 & $\star$ \\
\hline

 & 70985 & 20478 & 163578 & 51435 & 791.3 & 92.61 & 197.2 & $\circ$$\circ$$\circ$ \\* 
 & 45361 & 12912 & 92685 & 27352  & 323.7 & 99.46 & 208.9 & $\circ$$\circ$$\circ$ \\*
\cline{2-9}
 & 122378 & 35356 & 157131 & 45587 & 210.4 & 151.8 & 198.4 & $\circ$ \\* 
\multirow{-4}{*}{\tt brock400\_2}  & 82234 & 23157 & 95762 & 25701 & 210.8 & 166.8 & 214.9 & $\circ$ \\
\hline

\rowcolor[gray]{.8}  & 127946 & 39572 & 119906 & 37436 & 1308 & 146.8 & 143.9 & -- \\* 
\rowcolor[gray]{.8}  & 75133 & 21945 & 66964 & 19342  & 510.1 & 162.5 & 153.8 & $\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 168342 & 50294 & 113363 & 34720 & 332.0 & 193.2 & 133.6 & $\star$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt brock400\_3}  & 105186 & 29763 & 69544 & 20137 & 342.9 & 216.9 & 146.7 & $\star$ \\
\hline

 & 60763 & 17870 & 65939 & 20557 & 696.5 & 74.73 & 81.08 & $\circ$ \\* 
 & 35907 & 9813 & 36382 & 10389  & 270.3 & 81.78 & 85.50 & -- \\*
\cline{2-9}
 & 68010 & 19515 & 51187 & 15660 & 206.5 & 83.50 & 61.72 & $\star$ \\* 
\multirow{-4}{*}{\tt brock400\_4}  & 43000 & 11533 & 31194 & 8985 & 213.2 & 93.54 & 67.48 & $\star$ \\
\hline

\rowcolor[gray]{.8}  & 166590 & 42760 & 96961 & 24375 & 74323 & 649.4 & 403.3 & $\star$$\star$ \\* 
\rowcolor[gray]{.8}  & 92589 & 21232 & 54109 & 12126  & 2607 & 670.1 & 408.4 & $\star$$\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 306990 & 84282 & 151510 & 40865 & 2578 & 1173 & 622.0 & $\star$$\star$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt p\_hat700-3}  & 174538 & 43336 & 86027 & 20922 & 2296 & 1231 & 644.7 & $\star$$\star$ \\
\hline

 & 561752 & 195532 & 403867 & 141579 & -- & 970.4 & 727.8 & $\star$ \\* 
 & 297794 & 106338 & 227680 & 81421  & -- & 809.7 & 639.4 & $\star$ \\*
\cline{2-9}
 & 501918 & 173172 & 583655 & 205002 & 2361 & 899.3 & 1057 & $\circ$ \\* 
\multirow{-4}{*}{\tt frb30-15-1}  & 304227 & 106217 & 358024 & 128089 & 3057 & 824.4 & 961.4 & $\circ$ \\
\hline

\rowcolor[gray]{.8}  & 564777 & 196671 & 587228 & 205260 & -- & 967.5 & 1039 & $\circ$ \\* 
\rowcolor[gray]{.8}  & 323762 & 115112 & 337370 & 120645 & -- & 865.0 & 899.1 & -- \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 512867 & 183336 & 672671 & 240659 & 2725 & 897.5 & 1193 & $\circ$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt frb30-15-2}  & 323978 & 120593 & 436865 & 162446 & 2102 & 810.9 & 1052 & $\circ$ \\
\hline

 & 448754 & 156829 & 741805 & 268482 & -- & 779.7 & 1282 & $\circ$$\circ$ \\* 
 & 243166 & 87841 & 415467 & 156231  & -- & 652.5 & 1028 & $\circ$$\circ$ \\*
\cline{2-9}
 & 163409 & 59582 & 319548 & 121538  & 1551 & 294.2 & 557.2 & $\circ$$\circ$ \\* 
\multirow{-4}{*}{\tt frb30-15-3}  & 111497 & 41752 & 216080 & 84317 & 991.3 & 276.3 & 482.2 & $\circ$$\circ$ \\
\hline

\rowcolor[gray]{.8}  & 1781554 & 627424 & 843752 & 287111 & -- & 2961 & 1540 & $\star$$\star$ \\* 
\rowcolor[gray]{.8}  & 998141 & 364563 & 440556 & 153258  & -- & 2548 & 1259 & $\star$$\star$$\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 1125727 & 399811 & 483553 & 163851 & 4694 & 1905 & 901.6 & $\star$$\star$$\star$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt frb30-15-4}  & 753613 & 277360 & 297691 & 103577 & 3263 & 1746 & 789.2 & $\star$$\star$$\star$ \\
\hline

 & 664074 & 235213 & 995328 & 360589 & -- & 1170 & 1754 & $\circ$$\circ$ \\* 
 & 334927 & 123988 & 522826 & 198063 & -- & 897.5 & 1329 & $\circ$ \\*
\cline{2-9}
 & 342092 & 126432 & 623818 & 236143 & 3412 & 601.5 & 1075 & $\circ$$\circ$ \\* 
\multirow{-4}{*}{\tt frb30-15-5}  & 239928 & 91485 & 457648 & 177749 & 2166 & 546.5 & 963.2 & $\circ$$\circ$ \\
\hline

\rowcolor[gray]{.8}  & 11607 & 4539 & 10304 & 3998 & 315.0 & 14.69 & 13.18 & $\star$ \\* 
\rowcolor[gray]{.8}  & 3465 & 1439 & 2993 & 1233  & 44.69 & 13.67 & 12.28 & $\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 14729 & 5710 & 14528 & 5683 & 27.16 & 18.22 & 18.34 & -- \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt sanr200\_0.9}  & 6079 & 2367 & 5874 & 2325 & 21.60 & 20.76 & 20.66 & -- \\
\hline

 & 991805 & 388397 & 781787 & 302033 & 48193 & 1240 & 1183 & -- \\* 
 & 316861 & 131958 & 245797 & 100860 & 3550 & 1271 & 1032 & $\star$ \\*
\cline{2-9}
 & 1137737 & 445366 & 972115 & 378289 & 2361 & 1474 & 1303 & $\star$ \\* 
\multirow{-4}{*}{\tt C250.9}  & 459609 & 182377 & 390771 & 154130 & 1964 & 1666 & 1553 & $\star$ \\
\hline

\rowcolor[gray]{.8}  & 197.1 & 82.04 & 687.2 & 286.7 & 5.87 & 0.259 & 0.976 & $\circ$$\circ$$\circ$ \\* 
\rowcolor[gray]{.8}  & 66.56 & 30.46 & 205.6 & 93.02 & 0.512 & 0.218 & 0.891 & $\circ$$\circ$$\circ$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 329.5 & 146.1 & 966.1 & 427.7 & 0.766 & 0.432 & 1.39 & $\circ$$\circ$$\circ$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt gen200\_p0.9\_44}  & 142.2 & 66.60 & 361.4 & 167.3 & 0.493 & 0.437 & 1.22 & $\circ$$\circ$$\circ$ \\
\hline

 & -- & -- & 2364038 & 910227  & 6373176 & $>$ 18000 & 6289 &
 $\star$$\star$$\star$ \\* 
 & -- & -- & 666569 & 261728 & 63689 & $>$ 18000 & 3691 & $\star$$\star$$\star$
 \\* 
 \cline{2-9} & -- & -- & -- & -- & -- & $>$ 18000 & $>$ 18000 & -- \\* 
\multirow{-4}{*}{\tt gen400\_p0.9\_55}  & -- & -- & -- & -- & -- & $>$ 18000 & $>$ 18000 & -- \\
\hline

\rowcolor[gray]{.8}  & -- & -- & 536110 & 193972 & -- & $>$ 18000 & 1527 &
$\star$$\star$$\star$ \\* 
\rowcolor[gray]{.8}  & -- & -- & 116621 & 44894  & 165240 & $>$ 18000 & 749.1 & $\star$$\star$$\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & -- & -- & -- & -- & -- & $>$ 18000 & $>$ 18000 & -- \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt gen400\_p0.9\_65}  & -- & -- & -- & -- & -- & $>$ 18000 & $>$ 18000 & -- \\
\hline

 & 377.0 & 159.1 & 302.0 & 83.82 & 3.70 & 0.745 & 1.00 & $\circ$ \\* 
 & 52.64 & 26.83 & 28.50 & 9.85  & 0.109 & 0.340 & 0.312 & $\star$ \\*
\cline{2-9}
 & 5275 & 2194 & 30308 & 11794   & 60.44 & 13.36 & 71.00 & $\circ$$\circ$$\circ$ \\* 
\multirow{-4}{*}{\tt san400\_0.9\_1}  & 1957 & 909.4 & 5088 & 2170 & 15.54 & 8.58 & 32.82 & $\circ$$\circ$$\circ$ \\
\hline

\rowcolor[gray]{.8}  & 37.90 & 18.30 & 40.40 & 19.39 & 2.72 & 0.194 & 0.213 & $\circ$ \\* 
\rowcolor[gray]{.8}  & 8.92 & 4.67 & 9.94 & 5.32  & 0.872 & 0.123 & 0.139 & $\circ$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 37.90 & 18.30 & 40.40 & 19.39 & 0.453 & 0.178 & 0.198 & $\circ$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt MANN\_a27}  & 8.92 & 4.67 & 9.94 & 5.32 & 0.310 & 0.142 & 0.163 & $\circ$ \\
\hline

 & 2952 & 1081 & 3827 & 1485 & 3368 & 71.05 & 94.25 & $\circ$ \\* 
 & 242.9 & 118.7 & 452.9 & 225.6  & 306.2 & 18.40 & 31.73 & $\circ$$\circ$ \\*
\cline{2-9}
 & 2952 & 1081 & 3827 & 1485 & 220.7 & 63.46 & 84.82 & $\circ$ \\* 
\multirow{-4}{*}{\tt MANN\_a45}  & 242.9 & 118.7 & 452.9 & 225.6 & 53.16 & 18.10 & 39.18 & $\circ$$\circ$$\circ$ \\
\hline


==> nenem-leaves-grafos-dimacs.tex <==
{\tt p\_hat1000-1} & 1000 & 0.245 & 10 \\ 
{\tt p\_hat1500-1} & 1500 & 0.253 & 12 \\ 
{\tt p\_hat1000-2} & 1000 & 0.490 & 46 \\ 
{\tt DSJC1000.5} & 1000 & 0.500 & 15 \\ 
{\tt DSJC500.5} & 500 & 0.500 & 13 \\ 
{\tt p\_hat700-2} & 700 & 0.500 & 44 \\ 
{\tt sanr400\_0.5} & 400 & 0.500 & 13 \\ 
{\tt brock800\_1} & 800 & 0.650 & 23 \\ 
{\tt brock800\_2} & 800 & 0.650 & 24 \\ 
{\tt brock800\_3} & 800 & 0.650 & 25 \\ 
{\tt brock800\_4} & 800 & 0.650 & 26 \\ 
{\tt sanr400\_0.7} & 400 & 0.700 & 21 \\ 
{\tt p\_hat300-3} & 300 & 0.740 & 36 \\ 
{\tt brock200\_1} & 200 & 0.750 & 21 \\ 
{\tt brock400\_1} & 400 & 0.750 & 27 \\ 
{\tt brock400\_2} & 400 & 0.750 & 29 \\ 

{\tt brock400\_3} & 400 & 0.750 & 31 \\ 
{\tt brock400\_4} & 400 & 0.750 & 33 \\ 
{\tt p\_hat700-3} & 700 & 0.750 & 62 \\ 
{\tt frb30-15-1} & 450 & 0.820 & 30 \\ 
{\tt frb30-15-2} & 450 & 0.820 & 30 \\ 
{\tt frb30-15-3} & 450 & 0.820 & 30 \\ 
{\tt frb30-15-4} & 450 & 0.820 & 30 \\ 
{\tt frb30-15-5} & 450 & 0.820 & 30 \\ 
{\tt sanr200\_0.9} & 200 & 0.890 & 42 \\ 
{\tt C250.9} & 250 & 0.900 & 44 \\ 
{\tt gen200\_p0.9\_44} & 200 & 0.900 & 44 \\ 
{\tt gen400\_p0.9\_55} & 400 & 0.900 & 55 \\ 
{\tt gen400\_p0.9\_65} & 400 & 0.900 & 65 \\ 
{\tt san400\_0.9\_1} & 400 & 0.900 & 100 \\ 
{\tt MANN\_a27} & 378 & 0.990 & 126 \\ 
{\tt MANN\_a45} & 1035 & 1.000 & 345 \\ 


==> nenem-leaves-grafos-rand.tex <==
{\tt 5000\_10} & 5000 & 0.100 & 7 \\ 
{\tt 10000\_10} & 10000 & 0.100 & 7--8 \\ 
{\tt 15000\_10} & 15000 & 0.100 & 8 \\ 
{\tt 5000\_20} & 5000 & 0.200 & 9 \\ 
{\tt 1000\_30} & 1000 & 0.300 & 9 \\ 
{\tt 5000\_30} & 5000 & 0.300 & 12 \\ 
{\tt 1000\_40} & 1000 & 0.400 & 12 \\ 
{\tt 500\_50} & 500 & 0.500 & 13 \\ 
{\tt 1000\_50} & 1000 & 0.500 & 15 \\ 
{\tt 500\_60} & 500 & 0.600 & 17 \\ 
{\tt 300\_65} & 300 & 0.650 & 17 \\ 

{\tt 500\_65} & 500 & 0.650 & 19--20 \\ 
{\tt 300\_70} & 300 & 0.700 & 20 \\ 
{\tt 500\_70} & 500 & 0.700 & 22--23 \\ 
{\tt 200\_80} & 200 & 0.800 & 25--26 \\ 
{\tt 300\_80} & 300 & 0.800 & 28--29 \\ 
{\tt 200\_90} & 200 & 0.900 & 40 \\ 
{\tt 200\_95} & 200 & 0.950 & 60--62 \\ 
{\tt 300\_98} & 300 & 0.980 & 116--121 \\ 
{\tt 500\_994} & 500 & 0.994 & 263--270 \\ 
{\tt 1000\_998} & 1000 & 0.998 & 601--605 \\ 


==> nenem-leaves-rand.tex <==

\rowcolor[gray]{.8}  & 522.8 & 9.95 & 542.7 & 8.77 & 5.77 & 1.22 & 1.23 & -- \\* 
\rowcolor[gray]{.8}  & 521.9 & 9.86 & 542.0 & 8.73 & 3.59 & 1.24 & 1.25 & -- \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 532.4 & 10.91 & 555.9 & 10.72 & 2.89 & 1.25 & 1.26 & -- \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt 5000\_10}  & 531.4 & 10.80 & 555.3 & 10.66 & 3.28 & 1.27 & 1.29 & -- \\
\hline

 & 4707 & 673.4 & 5159 & 832.3 & 109 & 21.84 & 21.92 & -- \\* 
 & 4645 & 629.4 & 5128 & 812.7 & 65.40 & 21.98 & 22.04 & -- \\*
\cline{2-9}
 & 4833 & 688.9 & 5056 & 769.4 & 49.85 & 22.34 & 22.00 & -- \\* 
\multirow{-4}{*}{\tt 10000\_10}  & 4778 & 650.5 & 5014 & 740.1 & 51.59 & 22.50 & 22.15 & -- \\
\hline

\rowcolor[gray]{.8}  & 20829 & 2648 & 20553 & 3106 & 556.9 & 121.0 & 116.2 & -- \\* 
\rowcolor[gray]{.8}  & 18372 & 1825 & 18072 & 2369 & 356.4 & 120.3 & 116.5 & -- \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 21468 & 2631 & 22900 & 3290 & 284.3 & 124.0 & 123.3 & -- \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt 15000\_10}  & 19115 & 1857 & 20783 & 2711 & 290.2 & 123.6 & 123.7 & -- \\
\hline

 & 29361 & 1657 & 30267 & 1705 & 214.7 & 66.75 & 67.16 & -- \\* 
 & 28493 & 1526 & 29571 & 1582 & 150.4 & 69.22 & 70.12 & -- \\*
\cline{2-9}
 & 29663 & 1605 & 31406 & 1708 & 167.7 & 68.39 & 70.07 & -- \\* 
\multirow{-4}{*}{\tt 5000\_20}  & 28825 & 1481 & 30539 & 1584 & 186.8 & 70.74 & 72.86 & -- \\
\hline

\rowcolor[gray]{.8}  & 328.9 & 51.80 & 387.7 & 61.98 & -- & 0.273 & 0.313 & $\circ$ \\* 
\rowcolor[gray]{.8}  & 289.5 & 42.00 & 343.6 & 52.08 & -- & 0.316 & 0.358 & $\circ$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 345.5 & 50.80 & 396.4 & 59.59 & 0.986 & 0.286 & 0.320 & $\circ$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt 1000\_30}  & 308.5 & 42.14 & 355.4 & 50.57 & 1.12 & 0.328 & 0.364 & $\circ$ \\
\hline

 & 1229261 & 142458 & 1355238 & 159621 & 9448 & 3335 & 3538 & $\circ$ \\* 
 & 1104626 & 114531 & 1262710 & 141777 & 6341 & 3409 & 3622 & $\circ$ \\*
\cline{2-9}
 & 1268906 & 140585 & 1354901 & 152294 & -- & 3479 & 3607 & -- \\* 
\multirow{-4}{*}{\tt 5000\_30}  & 1151697 & 115171 & 1258607 & 133535 & -- & 3552 & 3696 & -- \\
\hline

\rowcolor[gray]{.8}  & 3727 & 768.7 & 3699 & 776.0 & 17.54 & 3.74 & 3.78 & -- \\* 
\rowcolor[gray]{.8}  & 3110 & 494.0 & 3059 & 497.8 & 14.38 & 4.21 & 4.14 & -- \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 3908 & 777.7 & 3906 & 794.6  & 12.33 & 3.91 & 3.98 & -- \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt 1000\_40}  & 3304 & 520.4 & 3289 & 538.8 & 13.93 & 4.40 & 4.36 & -- \\
\hline

 & 949.9 & 238.7 & 849.5 & 211.9 & 3.92 & 0.686 & 0.644 & $\star$ \\* 
 & 738.9 & 162.3 & 653.1 & 136.2 & 3.05 & 0.838 & 0.771 & $\star$ \\*
\cline{2-9}
 & 968.8 & 232.3 & 973.1 & 236.5 & 1.75 & 0.711 & 0.731 & -- \\* 
\multirow{-4}{*}{\tt 500\_50}  & 769.7 & 162.6 & 768.0 & 163.1 & 2.05 & 0.868 & 0.874 & -- \\
\hline

\rowcolor[gray]{.8}  & 75966 & 16108 & 74069 & 15553 & 430.5 & 87.07 & 87.25 & -- \\* 
\rowcolor[gray]{.8}  & 70375 & 15366 & 68292 & 14806 & 316.1 & 95.01 & 95.10 & -- \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 79196 & 16216 & 76319 & 15397 & 294.8 & 91.14 & 90.52 & -- \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt 1000\_50}  & 73931 & 15515 & 70916 & 14683 & 326.3 & 99.12 & 98.36 & -- \\
\hline

 & 11912 & 3134 & 11318 & 2965 & 68.67 & 10.42 & 10.32 & -- \\* 
 & 8649 & 1973 & 8140 & 1803  & 43.60 & 12.55 & 12.06 & -- \\*
\cline{2-9}
 & 13189 & 3363 & 12640 & 3216 & 28.96 & 11.57 & 11.51 & -- \\* 
\multirow{-4}{*}{\tt 500\_60}  & 9861 & 2216 & 9378 & 2063 & 32.74 & 13.90 & 13.47 & -- \\
\hline

\rowcolor[gray]{.8}  & 1205 & 360.6 & 1104 & 325.9   & -- & 0.931 & 0.935 & -- \\* 
\rowcolor[gray]{.8}  & 836.8 & 224.5 & 757.9 & 197.8 & -- & 1.15 & 1.09 & $\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 1397 & 405.3 & 1318 & 379.4   & -- & 1.07 & 1.05 & -- \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt 300\_65}  & 1008 & 264.4 & 942.9 & 242.4 & -- & 1.33 & 1.29 & -- \\
\hline

 & 65250 & 17831 & 62803 & 17193 & -- & 62.30 & 62.16 & -- \\* 
 & 50299 & 14163 & 47488 & 13239 & -- & 73.04 & 71.74 & -- \\*
\cline{2-9}
 & 72288 & 19074 & 72730 & 19320 & -- & 69.25 & 71.68 & -- \\* 
\multirow{-4}{*}{\tt 500\_65}  & 57809 & 15643 & 57619 & 15642 & -- & 80.83 & 82.29 & -- \\
\hline

\rowcolor[gray]{.8}  & 3726 & 1152 & 3067 & 932.2  & 25.07 & 3.04 & 2.67 & $\star$ \\* 
\rowcolor[gray]{.8}  & 2466 & 720.3 & 1925 & 519.3 & 13.08 & 3.79 & 3.25 & $\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 3881 & 1156 & 4234 & 1284   & 7.04 & 3.21 & 3.58 & $\circ$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt 300\_70}  & 2660 & 732.4 & 2917 & 831.1 & 7.88 & 4.00 & 4.39 & $\circ$ \\
\hline

 & 492014 & 143505 & 465416 & 135411 & 3562 & 521.4 & 512.1 & -- \\* 
 & 334038 & 97140 & 312075 & 89662  & 1677 & 597.0 & 582.6 & -- \\*
\cline{2-9}
 & 574019 & 162193 & 536902 & 151032 & 1427 & 610.6 & 594.2 & -- \\* 
\multirow{-4}{*}{\tt 500\_70}  & 412843 & 117343 & 381648 & 107110 & 1417 & 699.2 & 671.1 & -- \\
\hline

\rowcolor[gray]{.8}  & 1187 & 422.3 & 1172 & 424.5   & 13.40 & 0.971 & 0.976 & -- \\* 
\rowcolor[gray]{.8}  & 619.0 & 208.6 & 602.5 & 207.3 & 4.90 & 1.23 & 1.22 & -- \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 1469 & 511.8 & 1458 & 516.2   & 2.59 & 1.18 & 1.20 & -- \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt 200\_80}  & 833.0 & 274.4 & 820.7 & 275.8 & 2.75 & 1.54 & 1.55 & -- \\
\hline

 & 135194 & 46638 & 107192 & 36505 & 1377 & 143.5 & 120.7 & $\star$ \\* 
 & 69045 & 23123 & 52842 & 17118  & 429.4 & 161.3 & 132.8 & $\star$ \\*
\cline{2-9}
 & 169699 & 57512 & 152912 & 51628 & 296.6 & 180.1 & 170.4 & $\star$ \\* 
\multirow{-4}{*}{\tt 300\_80}  & 95146 & 31331 & 83660 & 27077 & 290.8 & 206.7 & 192.6 & $\star$ \\
\hline

\rowcolor[gray]{.8}  & 17527 & 6956 & 13913 & 5501 & 705.2 & 21.03 & 17.59 & $\star$ \\* 
\rowcolor[gray]{.8}  & 5738 & 2407 & 4493 & 1879  & 80.66 & 21.89 & 17.88 & $\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 22919 & 9091 & 20974 & 8393 & 51.89 & 27.85 & 26.33 & $\star$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt 200\_90}  & 9620 & 3885 & 8772 & 3573 & 41.38 & 32.52 & 30.39 & $\star$ \\
\hline

 & 13572 & 6072 & 8592 & 3778 & 1386 & 23.40 & 15.69 & $\star$ \\* 
 & 2811 & 1429 & 1666 & 836.1 & 64.31 & 18.99 & 12.06 & $\star$$\star$ \\*
\cline{2-9}
 & 13901 & 6515 & 9125 & 4211  & 126.6 & 25.00 & 17.25 & $\star$ \\* 
\multirow{-4}{*}{\tt 200\_95}  & 4563 & 2249 & 3016 & 1468 & 70.74 & 27.38 & 19.14 & $\star$ \\
\hline

\rowcolor[gray]{.8}  & 207249 & 101342 & 115876 & 55630 & 308379 & 868.2 & 513.8 & $\star$$\star$ \\* 
\rowcolor[gray]{.8}  & 16007 & 9236 & 9045 & 5174  & 2859 & 358.0 & 207.6 & $\star$$\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 181164 & 97100 & 72846 & 38568   & -- & 752.8 & 329.9 & $\star$$\star$$\star$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt 300\_98}  & 36249 & 21256 & 15543 & 9107 & -- & 926.6 & 401.8 & $\star$$\star$$\star$ \\
\hline

 & 9999 & 5460 & 5475 & 2867   & -- & 95.88 & 56.35 & $\star$$\star$ \\* 
 & 140.9 & 88.76 & 53.91 & 33.06 & 42.51 & 22.51 & 7.56 & $\star$$\star$$\star$ \\*
\cline{2-9}
 & 21386 & 15619 & 1055 & 723.0 & -- & 191.0 & 10.73 & $\star$$\star$$\star$ \\* 
\multirow{-4}{*}{\tt 500\_994}  & 710.0 & 512.7 & 113.7 & 81.42 & -- & 226.7 & 32.02 & $\star$$\star$$\star$ \\
\hline

\rowcolor[gray]{.8}  & 5002 & 3186 & 2491 & 1589 & -- & 153.8 & 78.99 & $\star$$\star$ \\* 
\rowcolor[gray]{.8}  & 9.61 & 7.40 & 6.04 & 4.49 & 50.14 & 12.82 & 9.46 & $\star$ \\*
\cline{2-9}
\rowcolor[gray]{.8}  & 13315 & 10803 & 5816 & 4841  & -- & 394.5 & 177.7 & $\star$$\star$$\star$ \\* 
\rowcolor[gray]{.8} \multirow{-4}{*}{\tt 1000\_998} & 185.8 & 151.2 & 92.64 & 75.04 & -- & 803.3 & 337.2 & $\star$$\star$$\star$ \\
\hline

